Fine-Grained Neural Network Explanation by Identifying Input Features with Predictive Information

One principal approach for illuminating a black-box neural network is feature attribution, i.e. identifying the importance of input features for the network's prediction. The predictive information of features is recently proposed as a proxy for the measure of their importance. So far, the predictive information is only identified for latent features by placing an information bottleneck within the network. We propose a method to identify features with predictive information in the input domain. The method results in fine-grained identification of input features' information and is agnostic to network architecture. The core idea of our method is leveraging a bottleneck on the input that only lets input features associated with predictive latent features pass through. We compare our method with several feature attribution methods using mainstream feature attribution evaluation experiments. The code is publicly available.

==> chapters/method_old.tex <==
\section{Methodology}
\subsection{Implementation (Input Attribution)}
Important notations:\\
X: input\\
R: latent representation (features)\\
Z: masked latent representation\\
Y: output\\
$\epsilon$: feature noise\\
$\lambda$: feature mask\\
$\epsilon_{GAN}$: input noise learned by generative adversarial model\\
$\lambda_{GAN}$: input mask learned by generative adversarial model\\
$\epsilon_{in}$: input noise (constructed manually, must be Gaussian noise)\\
$\lambda_{in}$: input mask learned by input IBA\\

\subsection{Information Bottleneck}
First we generate masked latent representation $Z$ using a masking scheme $Z=m(R,\epsilon,\lambda)$, where $\epsilon$ is a general noise for masking. Then we apply IB as optimization problem to solve an optimal latent mask $\lambda$:
\begin{equation}
  \max_{\lambda} I(Y,Z) - \beta I(R,Z)
\end{equation}

\subsection{Generative Adversarial Model}
The objective is to find a variable $Z_{GAN}$ at input level (outside NN) which can be considered as the
cause of Z, i.e. $P(f(Z_{GAN}))=P(Z)$, where function $f$ is the NN part before IB. To simplify the problem
we have 2 assumptions. First we assume that Z is a masked latent representation for specific input X rather than an arbitary X. Second assumption is that $Z_{GAN}$ can be constructed by using the same masking scheme, $Z_{GAN} = m(X, \epsilon_{GAN}, \lambda_{GAN})$. The objective can be represented by:
\begin{equation}
    \min_{\lambda_{GAN}} D(P(f(m(X, \epsilon_{GAN}, \lambda_{GAN}))), P(m(R, \epsilon, \lambda)))
\end{equation}
D is a distance metric for similarity.
\subsection{Information Bottleneck on Input}
The $Z_{GAN}$ learned from GAN is an noisy approximation of masked input and has no guarantee on correctness. Thus, we only use $Z_{GAN}$ to approximate the true masked input $Z_{in}$ in an input information bottleneck. The optimization goal is
\begin{equation}
        \max_{\Lambda} I(Y,Z_{in}) - \beta I(X,Z_{in}) \\
\end{equation}
where $\Lambda$ is the input mask. $I(X,Z_{in})$ can be calculated by
% \begin{equation}
%     \begin{aligned}
%         I(X,Z_{in}) &= E_X[D_{KL}[P(Z_{in}|X)||P(Z_{in})]] \\
%         P(Z_{in}|X) &= m(X, \epsilon_{in}, \Lambda) \\
%          P(Z_{in}) &= m(Z_{GAN}, \epsilon_{in}, \Lambda) \\
%     \end{aligned}
% \end{equation}
$$I(X,Z_{in}) &= E_X[D_{KL}[P(Z_{in}|X)||P(Z_{in})]]$$
where $P(Z_{in}|X)$ is the distribution of masked input $Z_{in}$ given input $X$, we can obtain $P(Z_{in}|X)$ by apply masking scheme on input constant X:
\begin{equation}
    \begin{aligned}
        P(Z_{in}|X) &= m(X, \epsilon_{in}, \Lambda) \\
        &= \mathcal{N}(\Lambda X + (1-\Lambda)\mu_{in}, (1-\Lambda)^2\sigma_{in}^2)
    \end{aligned}
\end{equation}
$Z_{in}$ denotes the distribution of the masked input, this variable is intractable to calculate since this require integrate $P(Z_{in}|X)$ over the whole input space X (similar as in IBA, calculate $P(Z)$ requires integrate $P(Z_|R)$ over hidden space R). To obtain an accurate estimate of $Z_{in}$ we leverage the result from generative model, which means we take $Z_{GAN}$ and apply the current input mask on it to form an estimate of $Z_{in}$. This can be described mathematically by:
\begin{equation}
    \begin{aligned}
        P(Z_{in}) &= m(Z_{GAN}, \epsilon_{in}, \Lambda)\\
        &= m(m(X, \epsilon_{in}, \lambda_{GAN}), \epsilon_{in}, \Lambda) \\
        &= \Lambda(\lambda_{GAN}X + (1-\lambda_{GAN})\epsilon_{in}) + (1-\Lambda)\epsilon_{in} \\
        &= \lambda_{GAN}\Lambda X + (1 - \lambda_{GAN}\Lambda)\epsilon_{in} \\
        &= \mathcal{N}(\lambda_{GAN}\Lambda X + (1 - \lambda_{GAN}\Lambda)\mu_{in}, (1 - \lambda_{GAN}\Lambda)^2\mu_{in}^2)\\
    \end{aligned}
\end{equation}
Now we can focus on calculating KL divergence with $P(Z_{in})$ and $P(Z_{in}|X)$. It is obvious that both $P(Z_{in})$ and $P(Z_{in}|X)$ are Gaussian distributions since input noise $\epsilon_{in}$ is a Gaussian noise, also we know for two Gaussian distributions $p(x)=\mathcal{N}(\mu_1, \sigma_1)$ and $q(x)=\mathcal{N}(\mu_2, \sigma_2)$, the KL divergence is
$$KL(p,q) = \log\frac{\sigma_1}{\sigma_2}+\frac{\sigma_1^2+(\mu_1-\mu_2)^2}{2\sigma_2^2}-\frac{1}{2}$$
We also apply mean field factorization:
$$q(Z) = q(z_1,..., z_m) = \sum^m_{j=1}q(z_j)$$
So we can calculate KL divergence in a simpler way since KL divergence is additive for independent distributions:
$$D_{KL}[P||Q]=\sum_{i=1}^N D_{KL}[P_i||Q_i]$$
Finally, for a single factor, the KL divergence is:
\begin{equation}
    \begin{aligned}
        &D_{KL}[P(Z_{in,i}|X_i)||P(Z_{in,i})] \\
        &= D_{KL}[\mathcal{N}(\Lambda X + (1-\Lambda)\mu_{in}, (1-\Lambda)^2\sigma_{in}^2) || \mathcal{N}(\lambda_{GAN}\Lambda X + (1 - \lambda_{GAN}\Lambda)\mu_{in}, (1 - \lambda_{GAN}\Lambda)^2\mu_{in}^2))] \\
        &= \log\frac{(1-\lambda_{GAN}\Lambda)\sigma_{in}}{1-\Lambda)\sigma_{in}} + \frac{(1-\Lambda)^2\sigma_{in}^2}{2(1-\lambda_{GAN}\Lambda)^2\sigma_{in}^2} \\
        &+ \frac{(\Lambda X+(1-\Lambda)\mu_{in}-(\lambda_{GAN}\Lambda X + (1-\lambda_{GAN}\Lambda)\mu_{in}))^2}{2(1-\lambda_{GAN}\Lambda)^2\sigma_{in}^2} -\frac{1}{2} \\
        &= \log\frac{1-\lambda_{GAN}\Lambda}{1-\Lambda} + \frac{(1-\Lambda)^2}{2(1-\lambda_{GAN}\Lambda)^2} + \frac{(X-\mu_{in})^2(\Lambda -\lambda_{GAN}\Lambda)^2}{2(1-\lambda_{GAN}\Lambda)^2\sigma_{in}^2} -\frac{1}{2} \\
    \end{aligned}
\end{equation}
Summing over all factors we get the KL divergence, then using Mount-Carlo estimate over X we obtain the mutual information $I(X, Z_{in})$
\subsection{Task Specific Implementation}
masking scheme (input, latent)\\
noise (input, latent)\\
mutual information calculation\\
loss function\\
discriminator\\
\subsection{Attribution in Computer Vision}
TODO
\subsection{Attribution in NLP}
To mask a text, we apply interpolation between the word in the text and a Gaussian noise with zero mean and standard deviation of 1. We use this noise since the word embedding we constructed during training also maps $<unk>$
token (the token for "unknown" word) to embedding space using this Gaussian noise. 

\subsection{Optimize I(Y,Z)}
The proof is based on the variational information bottleneck\cite{VIB}.

Proof: Here we want to prove that for per-sample Information Bottleneck under classification cases, optimizer of cross entropy loss can is also the optimal value for mutual information I(Y,Z) under some assumptions. First we assume $Y \leftrightarrow X \leftrightarrow Z$, this means that Y and Z are independent given X. This assumption is fulfilled by masking scheme and data generation process, for Z we have $Z=m(X, \epsilon, \lambda)$, thus Z depends on X given sampled noise and mask; for Y we have $Y=g(X)$, were function g represents the data generation process for the task, which assign label for all data. Based on that we have: $$p(x,y,z)=p(y|x,z)p(z|x)p(x)=p(y|x)p(z|x)p(x)$$
Thus we can also calculate $p(y|z)$ by:
$$p(y|z)=\frac{p(z,y)}{p(z)}=\int\frac{p(y|x)p(z|x)p(x)}{p(z)}dx$$
Proof below are based on (cite variational information bottleneck):
\begin{equation}
    \begin{aligned}
        I(Z,Y)&=\int p(y,z)\log\frac{p(y,z)}{p(y)p(z)}dydz\\
        &=\int p(y,z)\log\frac{p(y|z)}{p(y)}dydz\\
    \end{aligned}
\end{equation}
However, calculate $p(y|z)$ requires integral over x, which is intractable. We then apply the variational idea that approximate $p(y|z)$ by $q_{\theta}(y|z)$ instead. $q_{\theta}(y|z)$ represents the neural network part after bottleneck, $\theta$ indicates parameter of NN part.
\begin{equation}
    \begin{aligned}
        I(Z,Y)&=\int p(y,z)\log\frac{p(y,z)}{p(y)p(z)}\frac{q_{\theta}(y|z)}{q_{\theta}(y|z)}dydz\\
        &=\int p(y,z)\log\frac{q_{\theta}(y|z)}{p(y)}dydz + \int p(y,z)\log\frac{p(y|z)}{q_{\theta}(y|z)}dydz\\
        &=\int p(y,z)\log\frac{q_{\theta}(y|z)}{p(y)}dydz + \int p(z)D_{KL}[p(y|z)||q_{\theta}(y|z)]dz\\
        &=\int p(y,z)\log\frac{q_{\theta}(y|z)}{p(y)}dydz + \mathbb{E}_{z\sim p(z)}[D_{KL}[p(y|z)||q_{\theta}(y|z)]]\\
    \end{aligned}
\end{equation}
Since KL divergence is always non-negative, thus the second term is non-negative. 
\begin{equation}
    \begin{aligned}
        I(Z,Y)&\ge\int p(y,z)\log\frac{q_{\theta}(y|z)}{p(y)}dydz\\
        &=\int p(y,z)\log q_{\theta}(y|z)dydz - H(Y)\\
    \end{aligned}
\end{equation}
The second term $H(Y)$ is a constant and has no effect when optimize over mask. We can now further construct our optimization objective as $$\max_{\lambda} OE(Z,Y)$$\\
To get the final result, we first expand $p(y,z)$, then we construct an empirical data distribution $$p(x,y)=\frac{1}{N}\sum_{n=1}^N \sigma_{x_n}(x)\sigma_{y_n}(y)$$ Then we use reparameterization trick since $Z=f(x,\epsilon)$, and x is not a random variable. $$p(z|x)dz=p(\epsilon)d\epsilon$$
Combine all tricks together:
\begin{equation}
    \begin{aligned}
        OE(Z,Y)&=\int p(y,z)\log q_{\theta}(y|z)dydz\\
        &=\int p(y|x)p(z|x)p(x)\log q_{\theta}(y|z)dxdydz\\
        &=\frac{1}{N}\sum_{n=1}^N\int p(z|x_n)\log q_{\theta}(y_n|z)dz\\
        &=\frac{1}{N}\sum_{n=1}^N\int p(\epsilon)\log q_{\theta}(y_n|z)d\epsilon\\
        &=\frac{1}{N}\sum_{n=1}^N\mathbb{E}_{\epsilon\sim p(\epsilon)}[\log q_{\theta}(y_n|z)]\\
        &=\mathbb{E}_{\epsilon\sim p(\epsilon)}[\log q_{\theta}(y_{sample}|z)]\\
    \end{aligned}
\end{equation}
We can write the optimization problem as minimizing a loss function, then the loss function is
$$L=\mathbb{E}_{\epsilon\sim p(\epsilon)}[-\log q_{\theta}(y_{sample}|z)]$$
L is the cross entropy loss function for a single instance. After we find the optimizer, we now prove this optimizer is not only the optimizer for the lower bound function $OE(Y,Z)$, but also valid for mutual information$I(Y,Z)$ under per-sample setting. Now we consider the second term which we neglected during mutual information calculation:$$\mathbb{E}_{z\sim p(z)}[D_{KL}[p(y|z)||q_{\theta}(y|z)]]$$
This term equals zero if $p(y|z)\equiv q_{\theta}(y|z)$
\begin{equation}
    \begin{aligned}
        p(y|z)&=\frac{1}{N}\sum_{n=1}^N\frac{p(y|x_n)p(z|x_n)}{p(z)}\quad\quad\text{(single sample dataset)}\\
        &=\frac{p(y|x_{sample})p(z|x_{sample})}{p(z)}\\
        &=p(y|x_{sample})\\
    \end{aligned}
\end{equation}
$p(z|x_{sample})\equiv p(z)$ because we consider only one sample:
$$p(z) = \int p(z|x)p(x)dx\approx\frac{1}{N}\sum_{n=1}^N p(z|x_n)=p(z|x_{sample})$$
Now $p(y|z)\equiv q_{\theta}(y|z)$ can be easily proved, for $p(y|z)$:
\[
    p(y|z)=p(y|x_{sample})= 
\begin{cases}
    1,& \text{if } y=y_{sample}\\
    0,& \text{otherwise}
\end{cases}
\]
For $q_{\theta}(y|z)$, the optimizer maximize $\mathbb{E}_{\epsilon}[log(q_{\theta}(y_{sample}|z))]$. Then we have:
\[
    q_{\theta}(y|z)= 
\begin{cases}
    1,& \text{if } y=y_{sample}\\
    0,& \text{otherwise}
\end{cases}
\]
Thus they are equivalent, and the KL divergence is zero. As a result, we can remove the inequality in variational step.
